ExoTST: Exogenous-Aware Temporal Sequence Transformer for Time Series Prediction

Accurate long-term predictions are the foundations for many machine learning applications and decision-making processes. Traditional time series approaches for prediction often focus on either autoregressive modeling, which relies solely on past observations of the target ``endogenous variables'', or forward modeling, which considers only current covariate drivers ``exogenous variables''. However, effectively integrating past endogenous and past exogenous with current exogenous variables remains a significant challenge. In this paper, we propose ExoTST, a novel transformer-based framework that effectively incorporates current exogenous variables alongside past context for improved time series prediction. To integrate exogenous information efficiently, ExoTST leverages the strengths of attention mechanisms and introduces a novel cross-temporal modality fusion module. This module enables the model to jointly learn from both past and current exogenous series, treating them as distinct modalities. By considering these series separately, ExoTST provides robustness and flexibility in handling data uncertainties that arise from the inherent distribution shift between historical and current exogenous variables. Extensive experiments on real-world carbon flux datasets and time series benchmarks demonstrate ExoTST's superior performance compared to state-of-the-art baselines, with improvements of up to 10\% in prediction accuracy. Moreover, ExoTST exhibits strong robustness against missing values and noise in exogenous drivers, maintaining consistent performance in real-world situations where these imperfections are common.

==> sections_arxiv/backup.tex <==
\begin{abstract}
Prior forecasting approaches often overlook exogenous information, or "covariates," that are pertinent to predicting the current variable of interest, termed "endogenous". Modern transformer-based forecasting models address this issue by reframing it as a multivariate task, forecasting both exogenous and endogenous variables together as joint functions of their pasts, treating all variables equally. However, this method struggles to incorporate future exogenous information, often available and important for accurate forecasting. To address this limitation, we introduce FutureTST, a novel transformer-based framework designed to leverage future exogenous inputs for improved forecasting of endogenous variables in real-world systems. For the endogenous variable, we utilize patch-wise self-attention, which effectively captures the temporal relationships within the series. Additionally, we employ variate-wise cross-attention to bridge the influence of exogenous variable into endogenous variable thereby enhancing the model's ability to integrate and learn from external information. This dual attention mechanism allows FutureTST to dynamically adapt to internal and external input series changes, resulting in significantly improved forecast accuracy. Extensive experiments on multiple real-world datasets demonstrate that FutureTST outperforms existing time series forecasting approaches by 10\%, highlighting its effectiveness in utilizing external information for enhanced time series forecasting.
\end{abstract}

\begin{abstract}
Traditional time series forecasting methods, such as multivariate or univariate approaches, often fail to effectively incorporate valuable external information provided by exogenous drivers. To address this limitation, we introduce FutureTST, a novel transformer-based framework designed to leverage future exogenous drivers for improved forecasting of endogenous variables in real-world systems. For the endogenous variable, we utilize patch-wise self-attention, which effectively captures the temporal relationships within the series. Conversely, we employ variate-wise cross-attention for the exogenous variable that enhances the model's ability to integrate and learn from the external information. This dual attention mechanism allows FutureTST to dynamically adapt to changes in both the internal and external data streams, resulting in significantly improved forecast accuracy. Extensive experiments on various multiple datasets demonstrate that FutureTST outperforms existing transformer-based forecasting models in terms of accuracy, highlighting its effectiveness in utilizing external information for enhanced time series forecasting.
\end{abstract}


Transformer-based models \cite{vaswani2017attention} have emerged as a powerful alternative to LSTM models for time series modeling, offering several advantages. First, transformers excel at capturing long-term dependencies \cite{wu2021autoformer} in sequences because of their self-attention mechanism. This mechanism allows them to track different parts of the input sequence regardless of distance, effectively capturing long-term relationships between different time steps in a time series. Second, transformers are highly parallelizable \cite{dehghani2023scaling} and handle all input concurrently, whereas LSTMs process each input sequentially and, therefore, require more time to train. Lastly, transformers have demonstrated robustness to noise \cite{zhou2022understanding} and outliers in the input data. The self-attention mechanism enables the model to focus on relevant patterns and ignore irrelevant noise or anomalies, making it well-suited for real-world time series data that often contains noise and outliers \cite{angryk2020multivariate}. Because of these properties, transformer-based models have become prominent in time series \cite{liu2023itransformer, zhang2022crossformer, wu2023timesnet,nie2022time} forecasting and time-series-based foundational modeling \cite{ansari2024chronos,das2023decoder,liang2024foundation,yeh2023toward,rasul2023lag,darlow2023dam}, providing zero-shot capabilities for tasks entirely new to the model.






\section{Appendix}
\begin{table}[h]
\caption{Full results of the long-term forecasting with exogenous variables task.}
\vspace{2pt}
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.5}
\begin{sc}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|cc|cc|cc|cc|cc|cc|cc}
\toprule[1.2pt]  
\multicolumn{2}{c}{\multirow{2}{*}{\scalebox{1.35}{Models}}}   & \multicolumn{2}{c}{\scalebox{1.35}{FutureTST}} & \multicolumn{2}{c}{\scalebox{1.35}{(U) iTrans.}} & \multicolumn{2}{c}{\scalebox{1.35}{(M)iTrans.}} & \multicolumn{2}{c}{\scalebox{1.35}{(U)PatchTST}} & \multicolumn{2}{c}{\scalebox{1.35}{(M)PatchTST}} & \multicolumn{2}{c}{\scalebox{1.35}{LSTM}} & \multicolumn{2}{c}{\scalebox{1.35}{DLinear}} \\ 
\multicolumn{2}{c}{} & \multicolumn{2}{c}{\scalebox{1.35}{(Ours)}} & \multicolumn{2}{c}{\scalebox{1.35}{\citeyearpar{liu2023itransformer}}} & \multicolumn{2}{c}{\scalebox{1.35}{\citeyearpar{li2023revisiting}}} & \multicolumn{2}{c}{\scalebox{1.35}{\citeyearpar{nie2022time}}} & \multicolumn{2}{c}{\scalebox{1.35}{\citeyearpar{zhang2022crossformer}}} & \multicolumn{2}{c}{\scalebox{1.35}{\citeyearpar{das2023long}}}  & \multicolumn{2}{c}{\scalebox{1.35}{\citeyearpar{zeng2023transformers}}} \\ 
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){13-14}\cmidrule(lr){15-16}
\multicolumn{2}{c}{\scalebox{1.35}{Metric}}   & \scalebox{1.35}{MSE} & \scalebox{1.35}{MAE} & \scalebox{1.35}{MSE}    & \scalebox{1.35}{MAE}   & \scalebox{1.35}{MSE}    & \scalebox{1.35}{MAE}    & \scalebox{1.35}{MSE}    & \scalebox{1.35}{MAE} & \scalebox{1.35}{MSE}    & \scalebox{1.35}{MAE} & \scalebox{1.35}{MSE}    & \scalebox{1.35}{MAE}  & \scalebox{1.35}{MSE} & \scalebox{1.35}{MAE}         \\ 
\toprule[1.2pt]
\multirow{5}{*}{\scalebox{1.35}{\rotatebox{90}{ECL}}}     & \scalebox{1.35}{30} & \scalebox{1.35}{0.282} & \scalebox{1.35}{0.380} & 
\scalebox{1.35}{0.299} & \scalebox{1.35}{0.403} & 
\scalebox{1.35}{0.433} & \scalebox{1.35}{0.480}  & 
\scalebox{1.35}{\textbf{0.265}} & \scalebox{1.35}{\textbf{0.364}} & \scalebox{1.35}{0.405} & \scalebox{1.35}{0.459} & \scalebox{1.35}{0.342} & \scalebox{1.35}{0.437} & \scalebox{1.35}{0.387} & \scalebox{1.35}{0.451}   \\
& \scalebox{1.35}{60} & \scalebox{1.35}{0.319} & \scalebox{1.35}{0.399} 
&  \scalebox{1.35}{0.321} & \scalebox{1.35}{0.413} 
& \scalebox{1.35}{0.407} & \scalebox{1.35}{0.461} 
& \scalebox{1.35}{0.361} & \scalebox{1.35}{0.425} 
& \scalebox{1.35}{\textbf{0.313}} & \scalebox{1.35}{\textbf{0.390}} & \scalebox{1.35}{0.383} & \scalebox{1.35}{0.442} & \scalebox{1.35}{0.384} & \scalebox{1.35}{0.461}      \\
& \scalebox{1.35}{90} & \scalebox{1.35}{\textbf{0.362}} & \scalebox{1.35}{\textbf{0.429}}  & 
\scalebox{1.35}{0.379} & \scalebox{1.35}{0.446} & 
\scalebox{1.35}{0.440} & \scalebox{1.35}{0.481} & 
\scalebox{1.35}{0.393} & \scalebox{1.35}{0.440} & 
\scalebox{1.35}{0.380} & \scalebox{1.35}{0.431} & \scalebox{1.35}{0.418} & \scalebox{1.35}{0.464} & \scalebox{1.35}{0.439} & \scalebox{1.35}{0.493} \\
& \scalebox{1.35}{120} & \scalebox{1.35}{\textbf{0.380}} & \scalebox{1.35}{\textbf{0.450}}                & \scalebox{1.35}{0.461} & \scalebox{1.35}{0.504}                  & \scalebox{1.35}{0.495} & \scalebox{1.35}{0.523}            & 
\scalebox{1.35}{0.482} & \scalebox{1.35}{0.507}             & \scalebox{1.35}{0.418} & \scalebox{1.35}{0.463}                 & \scalebox{1.35}{0.471} & \scalebox{1.35}{0.507}          & \scalebox{1.35}{0.473} & \scalebox{1.35}{0.514}                        
\\ \cmidrule(lr){2-16}
& \scalebox{1.35}{AVG} & \scalebox{1.35}{\textbf{0.336}} & \scalebox{1.35}{0.414}                & \scalebox{1.35}{0.365} & \scalebox{1.35}{0.442}                  & \scalebox{1.35}{0.444} & \scalebox{1.35}{0.486}             & 
\scalebox{1.35}{0.394} & \scalebox{1.35}{0.446}              & \scalebox{1.35}{0.344} & \scalebox{1.35}{\textbf{0.412}}                 & \scalebox{1.35}{0.419} & \scalebox{1.35}{0.468}          & \scalebox{1.35}{0.410} & \scalebox{1.35}{0.476}

\\ \bottomrule[1.2pt]          

\end{tabular}}
\label{tab:full-log}
\end{sc}
\end{table}


\paragraph{Flux Tower Dataset}
encompasses key ecological and meteorological variables derived from ERA datasets and direct measurements, capturing precipitation, vapor pressure deficit, air temperature, and solar radiation and includes detailed assessments of ecosystem productivity through variables like Leaf Area Index and Gross Primary Production. This dataset is essential for modeling plant-environment interactions and understanding ecological dynamics across diverse biomes.

\textbf{Exogenous Drivers:} The following drivers are derived from ERA (European Reanalysis) datasets. 
\begin{enumerate}
    \item \textbf{Precipitation:} Precipitation data measures the amount of precipitation over a specific period and is useful for understanding water availability and hydrological cycles in the ecosystem.
    \item \textbf{VaporPressureDeficit:} Vapor Pressure Deficit is a measure of the difference between the amount of moisture in the air and how much moisture the air can hold when it is saturated. A higher VPD indicates drier air and can significantly influence plant transpiration rates and stress.
    \item \textbf{AirTemperature:} Air Temperature variable records the temperature of the air, which is fundamental in driving  biological and ecological processes.
    \item \textbf{SolarRadiation:} Shortwave Radiation Influx involves the measurement of incoming solar radiation and is critical for photosynthesis, evapotranspiration, and energy balance within the ecosystem.
    \item \textbf{LeafAreaIndex:} Leaf Area Index measures the total area of leaves per unit area of ground and is used to estimate the amount of foliage in an area, which in turn affects photosynthesis, transpiration, and energy absorption.
\end{enumerate}

\textbf{Endogenous Drivers:}
\begin{enumerate}
    \item \textbf{GrossPrimaryProductivity:} Gross Primary Production (GPP) is a measure of the amount of carbon dioxide captured by plants during photosynthesis and provide a fundamental indication of ecosystem productivity.
\end{enumerate}

\paragraph{CAMELS Dataset}
The \textbf{CAMELS} dataset, widely used in hydrological studies, includes a comprehensive set of exogenous meteorological drivers and records of hydrological responses as endogenous drivers. It is designed to support the modeling and analysis of water resources in diverse climatic conditions.

\textbf{Exogenous Drivers:}
\begin{enumerate}
    \item \textbf{Solar Radiation:} Measures the amount of solar energy reaching the ground, crucial for evaporation and plant photosynthesis processes.
    \item \textbf{Precipitation:} Records the total amount of rainfall and snowfall, vital for understanding water input into catchments.
    \item \textbf{Daylight Duration:} Duration of sunlight per day, affecting temperature and photosynthetic periods.
    \item \textbf{Snow Water Equivalent:} Represents the amount of water contained within the snowpack, critical for seasonal hydrological predictions.
    \item \textbf{Maximum Temperature:} The highest daily temperature, influencing evaporation rates and thermal dynamics of catchments.
    \item \textbf{Minimum Temperature:} The lowest daily temperature, important for modeling frost events and thermal impacts on water storages.
    \item \textbf{Vapor Pressure:} Measures the pressure exerted by water vapor in the air, influencing humidity and precipitation processes.
\end{enumerate}

\textbf{Endogenous Drivers:}
\begin{itemize}
    \item \textbf{Observed Discharge:} The measured water flow rate from rivers or streams, providing direct insight into the hydrological response of a catchment to environmental conditions and meteorological inputs.
\end{itemize}

\textbf{Standard Benchmark Dataset}:
We also conduct experiments on popular time series datasets:
(1) The Electricity Transformer Temperature (ETT): dataset (ETTh1, ETTh2, ETTm1, ETTm2) encompasses two years of electric power data from two counties in China, with recordings on an hourly (H) and minute (m) basis. Each data point includes an "oil temperature" measurement and six power load features categorized by usage frequency and intensity: High Usage Frequency Load (HUFL), High Usage Low Load (HULL), Medium Usage Frequency Load (MUFL), Medium Usage Low Load (MULL), Low Usage Frequency Load (LUFL), and Low Usage Low Load (LULL). Each of these features is recorded at the hour level.
(2) Electricity: dataset consists of hourly electricity consumption records (in kWh) for 321 clients over a period of three years. We analyze the electricity consumption of the last client as the endogenous variable and consider the consumption data from the remaining 320 clients as exogenous variables.
(3) Traffic: The dataset includes hourly data on road occupancy rates (ranging from 0 to 1) collected by 862 sensors across the San Francisco Bay Area freeways from 2015 to 2016, covering a total of 48 months. We consider the measurements from the last sensor as the endogenous variable while treating the data from the other 861 sensors as exogenous variables.
(4) Exchange: The dataset comprises daily exchange rates for eight foreign countries—Australia, Britain, Canada, Switzerland, China, Japan, New Zealand, and Singapore—spanning from 1990 to 2010. We treat the exchange rates of seven countries as exogenous variables and the exchange rate of one country as an endogenous variable.
(5) Influenza-like illness (ILI):  This dataset includes national weekly data on influenza cases collected by the CDC from 2002 to 2020. It tracks the total patients with respiratory symptoms (endogenous) across the country and includes external factors (exogenous) like influenza-like illness ratio measured in two ways (weighted and unweighted), number of cases in different age groups (0-4 years and 5-24 years), and the total number of Influenza cases. It also records how many healthcare providers reported these figures.
(6) Weather: The dataset includes recordings from the Weather Station of the Max Planck Institute for Biogeochemistry, capturing 21 meteorological indicators every 10 minutes throughout the entire year of 2020. These indicators include air temperature, humidity, and other factors. In our analysis, we use the Wet Bulb temperature as the endogenous variable to be predicted, while treating the remaining meteorological indicators as exogenous variables.


==> sections_arxiv/introduction_old.tex <==
\section{Introduction}






% Why transformer-based models over LSTM-based models? 

Accurate long-term forecasting is crucial across various fields, including climate sciences, finance, and biomedicine. In recent years, Deep learning models, such as Transformer \cite{vaswani2017attention}, have become increasingly prominent in long-term time series forecasting \cite{liu2023itransformer, zhang2022crossformer, wu2023timesnet,nie2022time,wang2024timexer}. These models employ self-attention mechanisms that effectively focus on relevant long-term and short-term patterns while filtering out noise or anomalies, a feature particularly advantageous for processing real-world time series data \cite{angryk2020multivariate}. Consequently, transformer-based models have also been widely adopted for the development of foundational models for time series data \cite{ansari2024chronos,das2023decoder,liang2024foundation,yeh2023toward,rasul2023lag,darlow2023dam}, providing zero-shot capabilities for novel tasks.

 

In time series analysis, two prominent modeling approaches are the forward model (X$\to$Y) and the autoregresive model (Y$\to$Y). The forward model predicts the response (Y) based on its observed drivers (X), making it suitable for understanding the relationship between driver and response. In contrast, the autoregressive model (Y$\to$Y) predicts the future values of a time series (Y) based on its past values (Y), which is useful for capturing patterns, trends, and long-term dependencies. This approach leverages historical data to make predictions based on the characteristic of the variates being studied.
\begin{figure}[t]
        
    \includegraphics[width=1.05\linewidth]{images/new_patchtst.png}
    
    % \vspace{-8pt}
   \caption{\footnotesize We illustrate four distinct architectures used in Transformer-based models for time series forecasting, differentiated by their handling of endogenous (orange) and exogenous (white) data series.}
    \label{fig:Compare-Forecasting}
   
\end{figure}



Existing paradigms for time series forecasting primarily focus on autoregressive models, and they can be categorized into four categories, as illustrated in Figure \ref{fig:Compare-Forecasting}. The first category (Figure 1a) showcases models like PatchTST \cite{nie2022time} that perform univariate forecasting, i.e., they process each variate of the time series independently, without considering the relationships between different variates of the series and may overlook important interactions between variables. Next, we have multivariate forecasting (Figure 1b) methods like iTransformer \cite{liu2023itransformer} and crossformer \cite{zhang2022crossformer}, which address the limitations of univariate methods by capturing dependencies between different variates of the time series, multivariate forecasting can potentially lead to more accurate predictions. In many multivariate time series, some variates are considered exogenous and can act as drivers for the endogenous time series. This leads to the third category (Figure 1c) of methods like Vector Autoregressive (VAR) models \cite{sims1980macroeconomics} and more recent transformer approaches like TimeXer \cite{wang2024timexer} that focus on predicting endogenous variates with past observations of itself and past observations of other exogenous variables in the system. By incorporating external factors, this approach provides a more comprehensive understanding of interrelationships among variables, making it a specialized case of Figure 1b. However, this being a purely autoregressive approach limits its ability to be utilized in situations where the exogenous information can be used to model a forward function that uses past endogenous (response) and past, future exogenous (driver) to model future response. In many scientific applications, such as in earth sciences, this problem is often modeled using forward models that predict future endogenous variables based solely on future exogenous variables \cite{kratzert2018rainfall,nathaniel2023metaflux }. While these forward models utilize future exogenous information, they fail to utilize the available past context effectively.  For instance, when modeling the streamflow response of a hydrological catchment, it is insufficient to rely solely on current precipitation (driver). It's essential to also integrate past context, which encompasses information about previous precipitation and streamflow patterns, crucial for capturing the system's state, such as snowpack accumulation. Recognizing the limitations of previous approaches (1a, 1b, and 1c) and the potential of forward models, a fourth category of models(Figure 1d) like TiDE~\cite{das2023decoder} that leverages interactions among future exogenous, past exogenous, and past endogenous variables to predict future endogenous variables have emerged.  By incorporating the richer information available from past and future contexts, these models aim to provide more accurate and reliable predictions. Such methods are particularly valuable in scenarios where future exogenous information is essential and available, often in many forecasting problems in science and engineering. For, e.g. forecasting of Carbon Flux under different future climate conditions (where these future climate conditions are exogenous drivers). 



% TiDE\cite{} is one recent encoder-decoder MLP approach designed to handle the problem illustrated in Figure 1(d). This method works by stacking and flattening all past and future projected exogenous variables, then concatenating them with past endogenous time series data to be processed by a dense encoder. The encoded embedding is then passed to the dense decoder output of which is then concatenated with the future projected exogenous variables and passed to the temporal decoder.

% TiDE \cite{} is one recent encoder decoder MLP approach that handles the problem shown in 1(d). by stacking and flattening all the past and future projected exogenous and concatenating them with past endogenous time series to be passed to to its encoder and flattening all the past and future projected exogenous and concatenating them to the encoded output to be passed to temporal decoder.

TiDE\cite{} is one recent encoder-decoder MLP approach designed to handle the problem illustrated in Figure 1(d).  It accomplishes this by incorporating both past endogenous and past and future exogenous variables. Initially, TiDE stacks and flattens past and future exogenous variables, concatenating them with past endogenous data. This combined input undergoes processing by a dense encoder, followed by a dense decoder. The output of the dense decoder is then concatenated with future exogenous variables to be fed to the temporal decoder. This method effectively utilizes past endogenous and exogenous variables to forecast future outcomes, thereby improving forecasting accuracy by capturing intricate relationships within the time series data. However, a significant challenge in this approach is the alignment of time series data. Both the endogenous and exogenous series must be synchronized in terms of their time stamps. Misalignment can lead to inaccuracies in the model's output, as the concatenated data may not correctly represent temporal data relationships. 
Apart from time alignment, ensuring that the data from different sources are synchronized in terms of frequency is challenging. For instance, exogenous data might be available daily, while endogenous data could be collected hourly. Resampling and transforming these datasets without losing important information is a critical and often complex task. Moreover, forecast reliability depends significantly on the quality and completeness of the exogenous data. Issues such as missing values, measurement errors, or inconsistencies in data collection methods can adversely affect the model's accuracy. Ensuring the continuous availability of quality exogenous data can be challenging, especially for real-time forecasting applications.



A widely used transformer-based method for forecasting is PatchTST \cite{nie2022time}, which treats segments of time series data as tokens, akin to words in language modeling. TPatch-based self-attention methods, like PatchTST, offer promising solutions to overcome some of the limitations of MLP-based approaches such as TiDE.  These methods have the advantage of capturing long-range dependencies more effectively and handling variable-length sequences more naturally. By attending to relevant patches of the input sequence, patch-based self-attention methods can better capture complex temporal patterns and relationships within the time series data. Additionally, they can adapt to varying patterns and frequencies within the data without the need for explicit alignment or resampling. This makes them more robust to irregularities and fluctuations in the data, ultimately improving forecasting accuracy and reliability.
Similarly, more recent approaches, like iTransformer \cite{liu2023itransformer}, can also similarly overcome these limitations in MLP-based models like the tide by viewing entire series as tokens and using self-attention between variates, enhancing the understanding of variable interrelationships. 
However, models like PatchTST and iTransformer often ignore exogenous factors important for accurate prediction of endogenous targets. These models typically address this issue by framing forecasting as a multivariate problem, equally considering both exogenous and target variables based solely on historical data.  This approach often falls short in practical scenarios, such as climatology, where leveraging projected future exogenous drivers is crucial for precise forecasting under different climate projections or scenarios. For example, forecasting Gross Primary Production (GPP)---the measure of carbon dioxide absorbed by vegetation through photosynthesis---heavily depends on future external climatic factors like precipitation, air temperature, and solar radiation, rather than just past GPP data. 


% These factors are readily forecasted by well-established physics-based earth system models, such as European Centre for Medium-Range Weather Forecasts Integrated Forecasting System (IFS) \cite{wedi2015modelling} and the Global Ensemble Forecast System (GEFS) \cite{zhou2022development}. Figure \ref{fig:driver_response_motivation} 

% \begin{figure}[t]
    
%    \centering
%     \begin{adjustbox}{center, addcode={\hspace*{+1.8cm}}{}} 
%         \includegraphics[width=1.5\linewidth]{images/patchtst.drawio.png}
%     \end{adjustbox}

%     % \vspace{-8pt}
%    \caption{\footnotesize (a) Existing transformer (TS)-based methods typically formulate the forecasting as a multivariate problem where both covariate and target variables are treated equally; (b) Our method, `FutureTST' utilizes both past and future multivariate exogenous drivers to forecast endogenous series.}
%     \label{fig:Compare-Forecasting}
   
% \end{figure}


\begin{figure*}[!t]
	\centering
	\begin{subfigure}[t]{0.49\textwidth}
		\centering
		\begin{overpic}[width=1\textwidth]{images/streamflow_motivation.png} 
		\end{overpic}		
		
		\caption{\small Hydrological Response}\label{fig:hydrology_response}
	\end{subfigure}
	~
	\begin{subfigure}[t]{0.49\textwidth}
		\centering
			
		\begin{overpic}[width=1\textwidth]{images/gpp_motivation.png} 
		\end{overpic}
  % \vspace{+0.32cm}			
	\captionsetup{justification=justified}
         \caption{\small Ecosystem Carbon Response }\label{fig:gpp_response}
           
	\end{subfigure}%\vspace{-0.2cm}
	
	\caption{\small The left figure illustrates the relationship between streamflow and rainfall, showing that streamflow levels increase following significant rainfall events. The right figure demonstrates how changes in air temperature influence the carbon cycle.}
	\label{fig:driver_response_motivation}
\end{figure*}

% For instance, when these earth system model predict conditions like higher solar radiation and temperature with plentiful precipitation, plants are typically expected to photosynthesize more, leading to higher GPP. Conversely, less favorable conditions result in lower GPP.  Recognizing and effectively integrating these external influences into forecasting models is crucial for achieving accurate and reliable predictions. 

%talk about the shortcomings of existing time series transformer-based architecture and how exogenous drivers play an important role. Describe how we have endogenous and exogenous drivers in weather applications and explain them in one line. 



% In various domains, such as weather \cite{wu2023interpretable, zhang2023skilful}, electricity market \cite{weron2014electricity}, transportation \cite{lv2014traffic}, time series forecasting is extensively being utilized for generating insights. As shown in Figure \ref{fig:Compare-Forecasting}, existing forecasting paradigms can be summarized into two distant categories. Compared with univariate and multivariate forecasting, forecasting with information about future exogenous variables introduces auxiliary information that can facilitate the endogenous variable's forecasting. Exogenous variables are prevalent and critical in practical applications since external factors,
% such as atmospheric conditions, geographical features, and human activities, often influence the variations within time series data. For instance, streamflow forecasting is highly dependent on various external factors like temperature, humidity, wind speed, and pressure, and it is not possible to predict future streamflow solely based on historical data. Incorporating external factors allows for a more comprehensive understanding of the interrelationships and causality among various variables, leading to better and more reliable performance. 



Integrating exogenous variables into the prediction models of endogenous variable introduces considerable computational challenges. First, it is essential to accurately capture the relationship between endogenous and exogenous variables, requiring the development of models adept at handling their interactions and dependencies. Second, the exogeneous drivers may present issues such as missing data, varying series length, or noisy data, demanding robust model designs that can accommodate these irregularities. Third, since exogenous variables often derive from dynamic projections, they are inherently noisy. Our model must be resilient against the noises in these exogenous drivers to reliably enhance our predictions. 


In this work, we overcome these challenges by drawing inspiration from multimodal models that learn joint representations of text, images, and videos. These models utilize a combination of cross-attention and self-attention mechanisms to project insights from one modality into another, facilitating a better understanding across diverse data types. Building on these concepts, we introduce EATST, an Exogenous-Aware Temporal Sequence
Transformer that integrates exogenous past and future drivers as distinct modalities while treating endogenous variables as a third modality. Within our framework, we implement patch-wise self-attention to effectively capture temporal relationships in both endogenous and exogenous variables. EATST comprises two encoders dedicated to processing past and future exogenous modalities and a decoder for the endogenous target series. A cross-temporal fusion module facilitates efficient information exchange between past and future exogenous encodings through cross-attention over aggregate tokens. Subsequently, the endogenous decoder incorporates the fused exogenous information and past endogenous values via cross-attention to generate future forecasts. By explicitly modeling future drivers and cross-modal interactions, EATST can leverage available future context more effectively, resulting in significantly improved forecasting accuracy in real-world systems. Our contributions are summarized below:



\begin{itemize}
    \item In this paper, we propose FutureTST, a novel framework designed for long-term forecasting of time series data, particularly in scenarios involving exogenous drivers. By incorporating these exogenous drivers, FutureTST systematically captures and integrates external influences into the forecasting model, enhancing prediction accuracy.    
    \item Experiments on real-world flux tower datasets show that FutureTST outperform extensive existing forecasting methods by 10\%. Additionally, our visualization of cross-attention maps indicates that FutureTST is able to identify key exogenous drivers consistent with our physical understanding, enhancing the scientific interpretability. 
\end{itemize}

==> sections_arxiv/old_methodology.tex <==
\section{Our approach: FutureTST}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/FutureTST.png} % Adjust width as needed
 
    \caption{\footnotesize Schematic illustration of the FutureTST model.
    } % Adjust font size as needed
    \label{fig:FutureTST}
  
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{images/foo.png} % Adjust width as needed
    \captionsetup{justification=centering, margin=0cm, font=footnotesize}
    \caption{\footnotesize MSEs of our FutureTST and the seven baseline models are compared across increasing forecasting horizons (30, 60, 90, and 120 days) at three sites for the test data. } % Adjust font size as needed
    \label{fig:graph}
    
\end{figure*}

In our proposed model framework (see Figure \ref{fig:FutureTST}), we use  Transformer based architecture, as they are known for their effectiveness in dealing with sequences and complex data dependencies. Our framework has an encoder-decoder architecture where the encoder is used to process exogenous weather drivers, and its encoded output is used by the decoder along with endogenous series to generate endogenous forecasts.  As the overall relationships across the exogenous drivers are  more significant than the individual data points, for the encoder, we use time encoding for the whole series, also called variate embedding, which focuses on capturing the broader pattern among the external factors. For endogenous variables,  every individual value is important. Hence, patch embedding is used to preserve the significance of each data point before feeding into the decoder block. Initially, the model, both encoder and decoder, use a self-attention mechanism for both types of data. 
% This allows it to learn the dependencies within each series on its own—capturing the data's order over time (temporal dependencies) and relationships among different variables (variate dependencies). 
Following this, the decoder uses a cross-attention step where the model uses the endogenous encodings as queries and the exogenous encoding as keys and values. This setup allows the model to integrate the influence of exogenous variables into endogenous variables. 


 
% Given that we are interested in the broader relationship of exogenous drivers, to capture exogenous embedding, we use whole time series as a variate token to capture multivariate correlation as done by recent work of iTransformer \cite{liu2023itransformer}. 

% Using whole time series as variate tokens allows the self-attention module to consider the entire temporal context and dependencies of the exogenous variables. It enables the model to learn the intricate patterns and correlations between the exogenous drivers and the target time series, potentially leading to improved forecasting performance and a better understanding of the underlying relationships.


\textbf{Exogenous Encoding}: Given that we are interested in the broader relationship of exogenous drivers, we propose using series-level representations \cite{liu2023itransformer} and applying self-attention to learn temporal dependencies between covariates. This approach involves embedding each exogenous series into a fixed-dimensional vector space using trainable linear projectors. By doing so, the model efficiently captures the overall dynamics and interactions between different exogenous variables, regardless of their lengths or any missing data points. This embedding strategy offers flexibility and robustness in handling challenges such as misaligned sampling periods and noise in the exogenous series. 


\textbf{Endogenous Patching}: To accurately forecast the endogenous variable, it is essential to consider the temporal dependencies within the data. Therefore, we adopt a representation that divides the endogenous series into overlapping segments similar to \cite{nie2022time}, where each segment is mapped to a unique temporal token through a trainable patch embedding module.
% The patch embedding module processes these patches of length $P$, transforming them into a $D$-dimensional space using a trainable linear projection and a position embedding. 
 

\textbf{Modality Fusion}
We employ cross-attention for variate modality fusion to capture the relationships between endogenous and exogenous variables. The endogenous variable serves as the query, while the exogenous embedding acts as the key and value.  This allows the multivariate correlations learned by the exogenous variate embedding to propagate to the endogenous temporal tokens, facilitating information transfer between the two types of modalities, as is commonly used in multi-modal learning approaches. Finally, a linear projection is applied to the decoder output to generate predictions for the endogenous variables. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/visualization.png} % Adjust width as needed
   
    \caption{\footnotesize Visualization of learned self-attention and cross-attention maps alongside endogenous look-back window for interpretation. } % Adjust font size as needed
    \label{fig:visualization}
    \
\end{figure}
